A Roadmap to Pluralistic Alignment

With increased power and prevalence of AI systems, it is ever more critical that AI systems are designed to serve all, i.e., people with diverse values and perspectives. However, aligning models to serve pluralistic human values remains an open research question. In this piece, we propose a roadmap to pluralistic alignment, specifically using language models as a test bed. We identify and formalize three possible ways to define and operationalize pluralism in AI systems: 1) Overton pluralistic models that present a spectrum of reasonable responses; 2) Steerably pluralistic models that can steer to reflect certain perspectives; and 3) Distributionally pluralistic models that are well-calibrated to a given population in distribution. We also formalize and discuss three possible classes of pluralistic benchmarks: 1) Multi-objective benchmarks, 2) Trade-off steerable benchmarks, which incentivize models to steer to arbitrary trade-offs, and 3) Jury-pluralistic benchmarks which explicitly model diverse human ratings. We use this framework to argue that current alignment techniques may be fundamentally limited for pluralistic AI; indeed, we highlight empirical evidence, both from our own experiments and from other work, that standard alignment procedures might reduce distributional pluralism in models, motivating the need for further research on pluralistic alignment.

==> experiementation.tex <==
% \begin{table*}[h]\centering
%     \resizebox{1\textwidth}{!}{
%     \begin{tabular}{ lccccccccc }\toprule
%         \multicolumn{1}{c}{\textbf{Model}}  & \multicolumn{3}{c}{LLaMA}  &\multicolumn{2}{c}{LLaMA2 (7B)} &\multicolumn{2}{c}{LLaMA2 (13B)} & \multicolumn{2}{c}{GPT-3}\\
        
%         \cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
        
%         \multicolumn{1}{c}{\textbf{Dataset}} & \textit{Pre} & \textit{Alpaca} & \textit{Tulu}  & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post}  \\
%         \midrule
%         GlobalQA (Japan)    & \textbf{0.40} & 0.45& 0.54&\textbf{0.47} &0.57 &\textbf{0.40} &0.55 &	&\\
%         GlobalQA (US)       & \textbf{0.38} & 0.41& 0.52&\textbf{0.43} &0.56 &\textbf{0.37} &0.53 &	&\\
%         MPI                 & \textbf{0.22} & 0.32& 0.48&\textbf{0.37} &0.51 &\textbf{0.42 }&0.46 & &	\\
%         \bottomrule
%     \end{tabular}}
%     % \vspace{-6pt}
%     \caption{Results comparing human distributions to model distributions on opinion multiple choice questions over two datasets, GlobalQA (target human distribution of Japan and US) and MPI. Each model class included comparison of models that are pre and post RLHF\footnote{Model detials, including exact models used, can be found in Appendix \ref{appx:exp_details}.}. Note that we compare two ``post" RLHF models for LLaMA (Alpaca and Tulu). }
%     \label{tab:toxicity_results}
%     % \vspace{-20pt}
% \end{table*}




% %ENTROPY!!
% \begin{table*}[h]\centering
%     \resizebox{1\textwidth}{!}{
%     \begin{tabular}{ lccccccccccccc }\toprule
%         \multicolumn{1}{c}{\textbf{Model}}  &   \multicolumn{2}{c}{Human} & \multicolumn{3}{c}{LLaMA}  &\multicolumn{2}{c}{LLaMA2 (7B)} &\multicolumn{2}{c}{LLaMA2 (13B)} & \multicolumn{2}{c}{GPT-3}\\
        
%         \cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
        
%         \multicolumn{1}{c}{\textbf{Dataset}}&  \textit{Japan/US} &\textit{Global} &\textit{Pre} & \textit{Alpaca} & \textit{Tulu}  & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post}  \\
%         \midrule
%         GlobalQA     & 0.96/0.99&NA& 1.38& 1.15& 0.67 & 1.20&0.61 & 1.19&0.51& & & \\
%         MPI              & NA  & 1.23& 1.40&1.02 & 0.78 &1.04 &0.65&  1.22 &0.73 & &	\\
%         \bottomrule
%     \end{tabular}}
%     % \vspace{-6pt}
%     \caption{Results comparing human distributions to \textit{shuffled} model distributions on opinion multiple choice questions over two datasets, GlobalQA (target human distribution of Japan and US) and MPI. Each model class included comparison of models that are pre and post RLHF\footnote{Model detials, including exact models used, can be found in Appendix \ref{appx:exp_details}.}. Note that we compare two ``post" RLHF models for LLaMA (Alpaca and Tulu). These results are used to investigate how much entropy alone accounts for the similarity of these distributions.}
%     \label{tab:toxicity_results}
%     % \vspace{-20pt}
% \end{table*}


%FINAL TABLES!!
% Original Models Similarity and Entropy

% \begin{table*}[htp]
% 
% \centering
%     \begin{tabular}{ lccccccccc }\toprule
%         \multicolumn{1}{c}{\textbf{Model Class}}  & \multicolumn{3}{c}{LLaMA}  &\multicolumn{2}{c}{LLaMA2 (7B)} &\multicolumn{2}{c}{LLaMA2 (13B)} & \multicolumn{2}{c}{GPT-3}\\
%         
%         \cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
%         
%         \multicolumn{1}{c}{\textbf{Dataset}} & \textit{Pre} & \textit{Alpaca} & \textit{Tulu}  & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post}  \\
%         \midrule
%         GlobalQA (Japan)    & \textbf{0.40} & 0.45& 0.54&\textbf{0.47} &0.57 &\textbf{0.40} &0.55 & \textbf{0.42} 	& 0.43\\
%         GlobalQA (US)       & \textbf{0.38} & 0.41& 0.52&\textbf{0.43} &0.56 &\textbf{0.37} &0.53 &\textbf{0.40} 	& 0.42 \\
%         MPI                 & \textbf{0.22} & 0.32& 0.48&\textbf{0.37} &0.51 &\textbf{0.42 }&0.46 & \textbf{0.41} & 0.44	\\
%         \bottomrule
%     \end{tabular}
%     % \vspace{-6pt}
%     \includegraphics[width=1\linewidth]{figurename}\\[1mm]
%   {A. Human Distribution vs. Model Distribution Similarity}
% 
% \bigskip
% 
%     \begin{tabular}{ lccccccccccccc }\toprule
%         \multicolumn{1}{c}{\textbf{Distribution}}  &   \multicolumn{2}{c}{Human} & \multicolumn{3}{c}{LLaMA}  &\multicolumn{2}{c}{LLaMA2 (7B)} &\multicolumn{2}{c}{LLaMA2 (13B)} & \multicolumn{2}{c}{GPT-3}\\
%         
%         \cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
%         
%         \multicolumn{1}{c}{\textbf{Dataset}}&  \textit{Japan/US} &\textit{Global} &\textit{Pre} & \textit{Alpaca} & \textit{Tulu}  & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post}  \\
%         \midrule
%         GlobalQA     & 0.96/0.99&NA& 1.38& 1.15& 0.67 & 1.20&0.61 & 1.19&0.51&  1.24 & 0.76 & \\
%         MPI              & NA  & 1.23& 1.40&1.02 & 0.78 &1.04 &0.65&  1.22 &0.73 & 1.41 & 0.90	\\
%         \bottomrule
%     \end{tabular}
%     % \vspace{-6pt}
%         \includegraphics[width=1\linewidth]{figurename}\\[1mm]
%   {B. Entropy}
%     \caption{Results comparing similarity (top) and entropy (bottom) of human distributions to model distributions on opinion multiple choice questions over two datasets, GlobalQA (target human distribution of Japan and US) and MPI. Each model class included comparison of models that are pre and post RLHF\footnote{Model detials, including exact models used, can be found in Appendix \ref{appx:exp_details}.}. Note that we compare two ``post" RLHF models for LLaMA (Alpaca and Tulu). In the top table, we bold the \textbf{smaller (more similar)} value.}
%     \label{tab:claim1}
% \end{table*}

   
% \begin{table*}[htp]
% 
% \centering
%     \begin{tabular}{ lccccccccc }\toprule
%         \multicolumn{1}{c}{\textbf{Model Class}}  & \multicolumn{3}{c}{LLaMA}  &\multicolumn{2}{c}{LLaMA2 (7B)} &\multicolumn{2}{c}{LLaMA2 (13B)} & \multicolumn{2}{c}{GPT-3}\\
%         
%         \cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
%         
%         \multicolumn{1}{c}{\textbf{Dataset}} & \textit{Pre} & \textit{Alpaca} & \textit{Tulu}  & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post}  \\
%         \midrule
%         GlobalQA (Japan)    & \textbf{0.40} & 0.45& 0.54&\textbf{0.47} &0.57 &\textbf{0.40} &0.55 & \textbf{0.42} 	& 0.43\\
%         GlobalQA (US)       & \textbf{0.38} & 0.41& 0.52&\textbf{0.43} &0.56 &\textbf{0.37} &0.53 &\textbf{0.40} 	& 0.42 \\
%         MPI                 & \textbf{0.22} & 0.32& 0.48&\textbf{0.37} &0.51 &\textbf{0.42 }&0.46 & \textbf{0.41} & 0.44	\\
%         \bottomrule
%     \end{tabular}
% 
%     \caption{Results comparing similarity (top) and entropy (bottom) of human distributions to model distributions on opinion multiple choice questions over two datasets, GlobalQA (target human distribution of Japan and US) and MPI. Each model class included comparison of models that are pre and post RLHF\footnote{Model detials, including exact models used, can be found in Appendix \ref{appx:exp_details}.}. Note that we compare two ``post" RLHF models for LLaMA (Alpaca and Tulu). In the top table, we bold the \textbf{smaller (more similar)} value.}
%     \label{tab:claim1}
% \end{table*}


% \begin{table}[htp]
% \centering
% \small % Adjust font size as necessary
% \begin{tabular}{ lccc }
% \toprule
% & GQA (Japan) & GQA (US) & MPI \\
% \midrule
% \textbf{LLaMA (Pre)}        & \textbf{0.40} & \textbf{0.38} & \textbf{0.22} \\
% Alpaca (Post)               & 0.45 & 0.41 & 0.32 \\
% Tulu (Post)                 & 0.54 & 0.52 & 0.48 \\
% \midrule
% \textbf{LLaMA2-7B (Pre)}    & \textbf{0.47} & \textbf{0.43} & \textbf{0.37} \\
% *-Chat (Post)          & 0.57 & 0.56 & 0.51 \\
% \midrule
% \textbf{LLaMA2-13B (Pre)}   & \textbf{0.40} & \textbf{0.37} & \textbf{0.42} \\
% *-Chat (Post)         & 0.55 & 0.53 & 0.46 \\
% \midrule
% \textbf{GPT-3 (Pre)}        & \textbf{0.42} & \textbf{0.40} & \textbf{0.41} \\
% GPT-3 (Post)                & 0.43 & 0.42 & 0.44 \\
% \bottomrule
% \end{tabular}
% \caption{Results comparing similarity (top) and entropy (bottom) of human distributions to model distributions on opinion multiple choice questions over two datasets, GlobalQA (target human distribution of Japan and US) and MPI. Each model class included comparison of models that are pre and post RLHF\footnote{Model details, including exact models used, can be found in Appendix \ref{appx:exp_details}.}. Note that we compare two ``post" RLHF models for LLaMA (Alpaca and Tulu). In the top table, we bold the \textbf{smaller (more similar)} value.}
% \label{tab:claim1}
% \end{table}




% %MODEL DISTR SHUFFLED!!
% \begin{table*}[h]\centering
%     \resizebox{1\textwidth}{!}{
%     \begin{tabular}{ lccccccccc }\toprule
%         \multicolumn{1}{c}{\textbf{Model Class}}  & \multicolumn{3}{c}{LLaMA}  &\multicolumn{2}{c}{LLaMA2 (7B)} &\multicolumn{2}{c}{LLaMA2 (13B)} & \multicolumn{2}{c}{GPT-3}\\
        
%         \cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
        
%         \multicolumn{1}{c}{\textbf{Dataset}} & \textit{Pre} & \textit{Alpaca} & \textit{Tulu}  & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post} & \textit{Pre} & \textit{Post}  \\
%         \midrule
%         GlobalQA (Japan)    & \textbf{0.45}& 0.51& 0.62&\textbf{0.51} &0.67 &\textbf{0.51} &0.68 & 	&\\
%         GlobalQA (US)       & \textbf{0.45}& 0.50& 0.62&\textbf{0.51} &0.66 &\textbf{0.51} &0.67 &	&\\
%         MPI                 & \textbf{0.34}& 0.47& 0.54&\textbf{0.50} &0.55 &\textbf{0.42 }&0.53 & &	\\
%         \bottomrule
%     \end{tabular}}
%     % \vspace{-6pt}
%     \caption{Results comparing human distributions to \textit{shuffled} model distributions on opinion multiple choice questions over two datasets, GlobalQA (target human distribution of Japan and US) and MPI. Each model class included comparison of models that are pre and post RLHF\footnote{Model detials, including exact models used, can be found in Appendix \ref{appx:exp_details}.}. Note that we compare two ``post" RLHF models for LLaMA (Alpaca and Tulu). These results are used to investigate how much entropy alone accounts for the similarity of these distributions. We bold the \textbf{smaller (more similar)} value.}
%     \label{tab:toxicity_results}
%     % \vspace{-20pt}
% \end{table*}
